An optimization-based construction procedure for function space based summation-by-parts operators on arbitrary grids

We introduce a novel construction procedure for one-dimensional summation-by-parts (SBP) operators. Existing construction procedures for FSBP operators of the form $D = P^{-1} Q$ proceed as follows: Given a boundary operator $B$, the norm matrix $P$ is first determined and then in a second step the complementary matrix $Q$ is calculated to finally get the FSBP operator $D$. In contrast, the approach proposed here determines the norm and complementary matrices, $P$ and $Q$, simultaneously by solving an optimization problem. The proposed construction procedure applies to classical SBP operators based on polynomial approximation and the broader class of function space SBP (FSBP) operators. According to our experiments, the presented approach yields a numerically stable construction procedure and FSBP operators with higher accuracy for diagonal norm difference operators at the boundaries than the traditional approach. Through numerical simulations, we highlight the advantages of our proposed technique.

==> 3_construction_old.tex <==
\section{Efficient Construction of operators} \label{sec:construction}
	In this section an algorithm is laid out to calculate an FSBP operator without explicitly prescribing more than a bare minimum of properties for the quadrature rule. This unlocks degrees of freedom that allow the calculation of banded FSBP operators. The conditions in definition \ref{def:wBFSBP} are equivalent to a set of convex constraints. To see this we define the auxiliary variables 
\begin{equation} \label{eq:RedSystem}
S = \frac{Q- Q^T}{2}, \quad W = \begin{pmatrix} V \\ - V_x \end{pmatrix} \in \R^{2N \times k}, \quad X = \begin{pmatrix} S & P \end{pmatrix} \in \R^{N \times 2N}.
\end{equation}
The matrix $S$ is the skew-symmetric part of $Q$ while $X$ combines the unknown variables into one matrix. 
Using these variables the definition above can be restated as
\begin{itemize}
	\item $Q = B/2 + S$. (SBP Property)
	\item $S$ is skew-symmetric. (SBP Property)
	\item $XW = -BV/2$ (Exactness)
	\item $\abs{k-l} > w \implies S_{kl} = 0$. (Operator is banded)
	\item $P_{kl} = P_{kk} \delta_{lk}$ (Diagonal P)
	\item $\sum_k P_{kk} = x_R - x_L$ (Quadrature is exact for constants)
	\item $P_{kk} > 0$ (Quadrature is positive)
\end{itemize}
\begin{remark}
	Multiplying $X$ and $W$ shows
	\[
		XW = SV - P V_x  = -BV/2 \implies (S + B / 2) V = P V_x \implies D_x V = V_x, 
	\]	
	i.e. the equivalence of the exactness condition in this definition and in the previous one.
\end{remark}
The main task is therefore reduced to calculating the matrix $X$ with the given restrictions on skew symmetry and positivity. Afterwards the components $S$ and $P$ that make up $X$ can be used to calculate the differentiation matrix $D$ as 
\[
Q = B/2  + S, \quad D = P^{-1} Q = P^{-1} B / 2 + P^{-1} S
\]
holds.
\begin{remark}
	The construction procedure above differs from the previous one, as previously the quadrature was determined first and the differentiation matrix $D_x$ was calculated afterwards in a second step. Here, we calculate both at the same time. This procedure is motivated by the fact that the quadratures are non-unique. If one calculates the quadrature first one could select a quadrature that satisfies the exactness conditions but is not compatible with the banded structure of $D_x$. By searching for the quadrature and the differentiation matrix $D_x$ at once we can evade this problem. 
	\end{remark}
	\begin{remark}
		The exactness of the quadrature for constants is part of the definition to allow proofs concerning shock-capturing capabilities of the resulting scheme when used in conjunction with suitable entropy corrections \cite{klein2023stabilizingII}. 
		\end{remark}
\subsection{A non-singular system of equations}
An interesting property lies in the fact that the matrix $W$ used in the construction above can be made orthogonal in the sense 
\[
	W^T \cdot W = \eye
\]
if discrete Sobolev orthogonal functions are used. These can be seen as a variation of Sobolev polynomials \cite{MX2015SOB, Marriaga2023SOB}.
\begin{definition}[Sobolev orthogonal functions]
	We call a set of functions $C = \{p_1, p_2, \dots \}$ Sobolev orthogonal if they are orthogonal with respect to the inner product of a Sobolev space, i.e.
	\[
		\forall i, j:\quad \skp[H^k] {p_i}{p_j} = \delta_{ij},
	\]
	where the inner product is of the form
	\[
		\skp[H^k]{p}{q} = \sum_{l=0}^{k} \skp{ \der [l] p x}{ \der [l] q x }.
	\]
	\end{definition}
	These are combined with the idea of discrete orthogonal polynomials.
	\begin{definition}[Discrete Orthogonal Functions]
		A set of functions $C = \{p_1, p_2, \dots \}$ shall be called discretely orthogonal if they are orthogonal 
		\[
				\forall i, j:\quad \dskp {p_i} {p_j} = \delta_{ij},
		\]
		with respect to an inner product based on discrete point evaluations
		\[
			\dskp{p}{q} = \sum_{m = 1}^n\sum_{l=1}^{n} p(x_m) G_{ml} q(x_l), \quad G \text{ pos. def.}
		\]
		\end{definition}
		If these Sobolev polynomials are now combined with a discrete inner product and applied to functions (not only polynomials) we arrive at the following definition.
		\begin{definition}[Discrete Sobolev Orthogonal functions]
				A set of functions $C = \{p_1, p_2, \dots \}$ shall be called discretely Sobolev orthogonal
			if they are orthogonal with respect to the inner product
			\[
				\dskp [H^k] {p}{q} = \sum_{j=0}^k \sum_{m = 1}^n\sum_{l=1}^{n} \der [j] p x (x_m) G_{j,ml} \der [j] p x (x_l), \quad G_j \in \R^{n\times n} \text{ pos. def.}
			\]
			\end{definition}
			\begin{lemma}
				Let $C = \left \{ p_1, p_2, \dots, p_j \right\}$ be discrete Sobolev orthonormal functions with respect to the $H^1$ inner product with $G_0 = \eye$ and $G_1 = \eye$. Then the matrix $W$ defined above in equation \eqref{eq:RedSystem} has pair-wise orthonormal columns.
				\end{lemma}
				\begin{proof}
					Calculating the inner product on $\R^n$ of two columns of the matrix $W$ results in 
					\[
						\left( W^T \cdot W \right)_{kl} = \sum_{m = 1}^n p_k(x_m) p_l(x_m) + \sum_{m = 1}^n \left(-\der {p_k} x (x_m)\right) \left(-\der {p_l} x (x_l)\right) = \dskp [H^1] {p_k}{p_l} = \delta_{kl}
					\]
					 \end{proof}
					 
			The result above allows us to calculate the Penrose inverse by using the transpose of $W$ when an orthonormal basis is used. We therefore propose the following algorithm to form a well posed system for the  operator from a given basis $ B =\{f_1, f_2, \dots f_j\}$ of the space $\mathcal{F} = \lspan B$.
			\begin{enumerate}
				\item Calculate a discrete Sobolev orthonormal function set $C = \{p_1, p_2, \dots, p_i\}$, $i \leq j$ out of $B$ using the Gram-Schmidt process \cite[Sec. 7 thm. 4]{Lax2007LA}
					\begin{equation}
					\begin{aligned}
						p_1 &= f_1 / \sqrt{\dskp[H^1] {f_1}{f_1}} \\ 
						\tilde p_k &= f_k  - \sum_{l=1}^{k-1} p_l \dskp[\mathrm{H^1}]{p_l}{f_k} \\ 
						p_k &= \frac{\tilde p_k}{\norm{\tilde p_k}_{\mathrm{H}^1}}
					\end{aligned}
					\end{equation}
				\item Assemble the matrices $V, V_x$ and $W$, initialize $X$ with zero.
				
			\end{enumerate}
			\subsection{Solving the problem with a quadratically convergent method}
			To find our operators we reformulate the problem as the following optimization problem
			\[
				\min_{X \in \Xi}  \norm{XW + BV / 2}^2
				\]
				suspect to the restriction that the matrix $X$ stems from the set
				\[
					\Xi =\left \{ X = \begin{pmatrix} S & P \end{pmatrix}\middle| S = -S^T \wedge P_{kl} = \delta_{kl} P_{kk} > 0 \wedge \sum_k P_{kk} = x_R - x_L\wedge \left(\abs{k-l} > w \implies S_{kl} = 0\right)\right \}.
				\]
				These restriction expresses that the quadrature is positive, exact for constants, the mass matrix diagonal and $S$ is skew-symmetric. 
				As we are in the field of large scale optimization we should try to evade the problems introduced by inequality constraints, as otherwise active set or projection methods would be needed. 
				\begin{remark}
						Projection methods are a usual technique for such optimization problems, but are only converging with first order. Therefore calculating the coefficients to near machine precision ($\epsilon \approx 10^{16}$) would need an excessive amount of iterations. Active set methods can be made quadratically convergent, but their complexity escalates with the number of variables and constraints. In our case a single step of such a method, that checks explicitly combinations of constraints that are active, would become impractically expensive.
				\end{remark}
				
				We will therefore reformulate our optimization problem via a parametrization $X : \R^L \to \Xi, \xi \mapsto X(\xi)$ that maps an unconstrained $L$-dimensional vector space to the set $\Xi$. One of these mappings is given by
				
				\[
				\begin{aligned}
					X((s, p)) = \begin{pmatrix} S(s) & P(p)  \end{pmatrix},& \quad S(s) = \begin{pmatrix}
						0 & s_1 & s_2 & 0&\dots\\
						-s_1 & 0 & s_3 & s_4 &\dots \\
						-s_2 & -s_3 & 0 & s_5 &\dots \\
						0 & - s_4 & -s_5 & 0 &\dots \\
						\vdots & \vdots & \vdots & \vdots& \ddots 
				 \end{pmatrix}, \\
			 \quad P(p) = (x_R - x_L) \begin{pmatrix} 
				 \sigma_1(p) & 0 & 0 & \dots \\
				 0 & \sigma_2(p) & 0 & \dots \\
				 0 & 0 & \sigma_3(p) & \dots \\
				 \vdots & \vdots & \vdots & \ddots
				 \end{pmatrix},&
			 \quad \sigma_k(p) = \frac{\e^{p_k}}{\sum_l \e^{p_l}}, 
			 \end{aligned}
				\]
				for an example bandwidth of $w = 2$ and we can therefore reformulate our optimization problem as the following unconstrained optimization problem
				\[
					\min_{(s, p) \in \R^N} \norm{X(s, p) W + BV / 2}^2.
				\]
				This optimization problem could be solved by gradient descent, but we observed that convergence rates are bad in this case. We assume that the reason for this are the spectral properties of the associated Hessian. 
				\begin{figure}
					\includegraphics[width=0.6\textwidth]{pygraphs/oscillationgd}
					\caption{Optimization problems with different length scales lead to gradients pointing nearly orthogonal away from the minimum. Therefore gradients are bad descent directions in this case. }
					\label{fig:GDbad}
				\end{figure} 
				If the optimization problem has a Hessian with rather large and small eigenvalues gradients will be bad directions for minimizing a functional in that direction, as depicted in figure \ref{fig:GDbad}.
				
				We therefore opt for the usage of second order optimization methods, i.e. methods that will not search for the optimum in the local direction of the steepest descent but try to build a quadratic model of the optimization landscape. Suitable examples are the nonlinear gradient descent and the limited memory BFGS method \cite{LN1989LBFGS,FR1964NLCG}.
				
				
			

==> csbpP.tex <==
\begin{equation}
P=\left[
\begin{array}{ccccccccc}
0.08854 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0.3073 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0.224 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0.2552 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0.25 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0.2552 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0.224 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.3073 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.08854 \\
\end{array}
\right]
\end{equation}


==> csbpQ.tex <==
\begin{equation}
Q=\left[
\begin{array}{ccccccccc}
-0.5 & 0.6146 & -0.08333 & -0.03125 & 0 & 0 & 0 & 0 & 0 \\
-0.6146 & 0 & 0.6146 & 0 & 0 & 0 & 0 & 0 & 0 \\
0.08333 & -0.6146 & 0 & 0.6146 & -0.08333 & 0 & 0 & 0 & 0 \\
0.03125 & 0 & -0.6146 & 0 & 0.6667 & -0.08333 & 0 & 0 & 0 \\
0 & 0 & 0.08333 & -0.6667 & 0 & 0.6667 & -0.08333 & 0 & 0 \\
0 & 0 & 0 & 0.08333 & -0.6667 & 0 & 0.6146 & 0 & -0.03125 \\
0 & 0 & 0 & 0 & 0.08333 & -0.6146 & 0 & 0.6146 & -0.08333 \\
0 & 0 & 0 & 0 & 0 & 0 & -0.6146 & 0 & 0.6146 \\
0 & 0 & 0 & 0 & 0 & 0.03125 & 0.08333 & -0.6146 & 0.5 \\
\end{array}
\right].
\end{equation}


==> csbpcoef.tex <==
\begin{equation}
\left[
\begin{array}{ccccccccc}
-5.647 & 6.941 & -0.9412 & -0.3529 & 0 & 0 & 0 & 0 & 0 \\
-2 & 0 & 2 & 0 & 0 & 0 & 0 & 0 & 0 \\
0.3721 & -2.744 & 0 & 2.744 & -0.3721 & 0 & 0 & 0 & 0 \\
0.1224 & 0 & -2.408 & 0 & 2.612 & -0.3265 & 0 & 0 & 0 \\
0 & 0 & 0.3333 & -2.667 & 0 & 2.667 & -0.3333 & 0 & 0 \\
0 & 0 & 0 & 0.3265 & -2.612 & 0 & 2.408 & 0 & -0.1224 \\
0 & 0 & 0 & 0 & 0.3721 & -2.744 & 0 & 2.744 & -0.3721 \\
0 & 0 & 0 & 0 & 0 & 0 & -2 & 0 & 2 \\
0 & 0 & 0 & 0 & 0 & 0.3529 & 0.9412 & -6.941 & 5.647 \\
\end{array}
\right]
\end{equation}


==> fsbpP.tex <==
\begin{equation}
P=\left[
\begin{array}{ccccccccc}
0.0788 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0.3432 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0.1873 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0.2349 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0.3117 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0.2349 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0.1873 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.3432 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.0788 \\
\end{array}
\right]
\end{equation}


==> fsbpQ.tex <==
\begin{equation}
Q=\left[
\begin{array}{ccccccccc}
-0.5 & 0.6136 & 0.005545 & -0.09575 & -0.07992 & 0.02095 & 0.04167 & 0.008644 & -0.01473 \\
-0.6136 & 0 & 0.3198 & 0.3079 & 0.1251 & -0.09406 & -0.08702 & 0.03314 & 0.008644 \\
-0.005545 & -0.3198 & 0 & 0.142 & 0.1949 & 0.06355 & -0.02978 & -0.08702 & 0.04167 \\
0.09575 & -0.3079 & -0.142 & 0 & 0.178 & 0.1858 & 0.06355 & -0.09406 & 0.02095 \\
0.07992 & -0.1251 & -0.1949 & -0.178 & 0 & 0.178 & 0.1949 & 0.1251 & -0.07992 \\
-0.02095 & 0.09406 & -0.06355 & -0.1858 & -0.178 & 0 & 0.142 & 0.3079 & -0.09575 \\
-0.04167 & 0.08702 & 0.02978 & -0.06355 & -0.1949 & -0.142 & 0 & 0.3198 & 0.005545 \\
-0.008644 & -0.03314 & 0.08702 & 0.09406 & -0.1251 & -0.3079 & -0.3198 & 0 & 0.6136 \\
0.01473 & -0.008644 & -0.04167 & -0.02095 & 0.07992 & 0.09575 & -0.005545 & -0.6136 & 0.5 \\
\end{array}
\right].
\end{equation}


==> fsbpcoef.tex <==
\begin{equation}
\left[
\begin{array}{ccccccccc}
-6.345 & 7.787 & 0.07037 & -1.215 & -1.014 & 0.2659 & 0.5289 & 0.1097 & -0.187 \\
-1.788 & 0 & 0.9321 & 0.8974 & 0.3645 & -0.2741 & -0.2536 & 0.09656 & 0.02519 \\
-0.0296 & -1.707 & 0 & 0.7583 & 1.04 & 0.3392 & -0.159 & -0.4645 & 0.2225 \\
0.4076 & -1.311 & -0.6048 & 0 & 0.7577 & 0.7912 & 0.2706 & -0.4004 & 0.08919 \\
0.2564 & -0.4013 & -0.6253 & -0.5709 & 0 & 0.5709 & 0.6253 & 0.4013 & -0.2564 \\
-0.08919 & 0.4004 & -0.2706 & -0.7912 & -0.7577 & 0 & 0.6048 & 1.311 & -0.4076 \\
-0.2225 & 0.4645 & 0.159 & -0.3392 & -1.04 & -0.7583 & 0 & 1.707 & 0.0296 \\
-0.02519 & -0.09656 & 0.2536 & 0.2741 & -0.3645 & -0.8974 & -0.9321 & 0 & 1.788 \\
0.187 & -0.1097 & -0.5289 & -0.2659 & 1.014 & 1.215 & -0.07037 & -7.787 & 6.345 \\
\end{array}
\right]
\end{equation}

